Learning Land-Surface Hydrology World Model from Satellite Observations

A world model should tell us not only what will happen, but what would happen under a different action. Learned Earth models now forecast remarkably well, yet forecast skill says little about what their state means or how it responds to a changed driver. We build LandWM, a world model of land-surface water in which rain is the action, learned from seven years of SMAP and CYGNSS observations: physical observation operators tie its latent state to soil water, and a mass-conserving balance governs how that state responds to rain. Over the U.S. Southern Great Plains, the model, never shown a soil-moisture value, tracks 28 in-situ probes as well as the operational SMAP Level-4 product, even from CYGNSS alone, and a storm added to the forcing of a station's cell wets its soil as natural storms wet the probes. Replace either piece and the forecasts stay, but the meaning goes: with neural operators, only a probe fitted to the stations finds the soil water; with a generic recurrent transition, rain on a single cell barely moves it. Yet when the same rain covers the whole region the two transitions swap roles, and the conserving one responds too weakly. Grounding makes a world model readable; its response to actions must be tested under more than one kind of intervention.

==> sec/6_llm.tex <==
\section*{LLM Usage Statement}
We used Claude Opus 5.5 (Anthropic) through Claude Code.
It wrote most of the code, ran the experiments, and drafted and polished the text; the research idea and all design decisions are the authors'.
All table numbers are generated by scripts from the experiment outputs, and the authors take full responsibility for the content.


==> tables/mm/twin.tex <==
% generated by code/scripts/make_twin_table.py -- do not edit by hand
\begin{tabular}{l cc cc c cc c}
\toprule
\rowcolor{tabhead}  & \multicolumn{2}{c}{Direct $R$} & \multicolumn{2}{c}{Probe $R$} & Assim. & \multicolumn{2}{c}{Rollout NLL} & Zero-rain \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){7-8}
\rowcolor{tabhead} Model & filter & rollout & filter & rollout & gain $\Delta R$ & SMAP & CYGNSS & SMAP NLL \\
\midrule
\rowcolor{tabours} \method & 0.72$\pm$0.04 & 0.78$\pm$0.04 & 0.74$\pm$0.05 & 0.76$\pm$0.03 & -0.003$\pm$0.008 & 4.26$\pm$0.03 & 1.52$\pm$0.01 & 9.95$\pm$0.23 \\
\quad neural decoder & 0.40 & 0.20 & 0.72 & 0.77 & 0.156 & 4.32 & 1.53 & 9.94 \\
\quad GRU transition & 0.77 & 0.80 & 0.74 & 0.77 & 0.006 & 4.17 & 1.53 & 10.28 \\
\quad black box & -0.22 & -0.26 & 0.73 & 0.76 & 0.019 & 4.18 & 1.52 & 10.22 \\
\rowcolor{tabbase} History Transformer & -- & -- & 0.65 & 0.69 & -- & 4.56 & 1.51 & 9.95 \\
\midrule
\rowcolor{tabbase} Rain-history ridge (no model) & -- & -- & 0.70$\pm$0.03 & 0.70$\pm$0.04 & -- & -- & -- & -- \\
\bottomrule
\end{tabular}


==> tables/mm/twin_cf.tex <==
% generated by code/scripts/make_twin_table.py -- do not edit by hand
\begin{tabular}{l cccc cccc}
\toprule
\rowcolor{tabhead}  & \multicolumn{4}{c}{Direct readout} & \multicolumn{4}{c}{Probe readout} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
\rowcolor{tabhead}  & \multicolumn{2}{c}{Rain effect} & \multicolumn{2}{c}{Drydown $\tau$} & \multicolumn{2}{c}{Rain effect} & \multicolumn{2}{c}{Drydown $\tau$} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
\rowcolor{tabhead} Model & $R$ & slope & median (d) & $\rho$ & $R$ & slope & median (d) & $\rho$ \\
\midrule
\rowcolor{tabours} \method & 0.97$\pm$0.00 & 0.98$\pm$0.06 & 3.2$\pm$0.6 & 0.93$\pm$0.01 & 0.97$\pm$0.00 & 0.89$\pm$0.00 & 2.8$\pm$0.3 & 0.90$\pm$0.00 \\
\quad neural decoder & 0.45 & 0.29 & 5.3 & 0.86 & 0.96 & 0.88 & 3.7 & 0.86 \\
\quad GRU transition & 0.97 & 1.21 & 3.0 & 0.98 & 0.98 & 0.95 & 3.3 & 0.98 \\
\quad black box & -0.23 & -0.13 & 7.8 & 0.32 & 0.97 & 0.95 & 3.2 & 0.96 \\
\rowcolor{tabbase} History Transformer & -- & -- & -- & -- & 0.86 & 0.75 & 3.5 & 0.91 \\
\midrule
\rowcolor{tabbase} Rain-history ridge (no model) & -- & -- & -- & -- & 0.77$\pm$0.04 & 0.54$\pm$0.02 & 2.8$\pm$0.5 & 0.36$\pm$0.11 \\
\midrule
\rowcolor{tabbase} Truth & 1 & 1.00 & 2.9$\pm$0.5 & 1 & 1 & 1.00 & 2.9$\pm$0.5 & 1 \\
\bottomrule
\end{tabular}


==> tables/ms/twin.tex <==
% generated by code/scripts/make_twin_table.py -- do not edit by hand
\begin{tabular}{l cc cc c cc c}
\toprule
\rowcolor{tabhead}  & \multicolumn{2}{c}{Direct $R$} & \multicolumn{2}{c}{Probe $R$} & Assim. & \multicolumn{2}{c}{Rollout NLL} & Zero-rain \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){7-8}
\rowcolor{tabhead} Model & filter & rollout & filter & rollout & gain $\Delta R$ & SMAP & CYGNSS & SMAP NLL \\
\midrule
\rowcolor{tabours} \method & 0.75$\pm$0.04 & 0.81$\pm$0.03 & 0.76$\pm$0.04 & 0.81$\pm$0.03 & -0.050$\pm$0.049 & 3.96$\pm$0.00 & 1.48$\pm$0.00 & 9.94$\pm$0.30 \\
\quad neural decoder & 0.25 & 0.00 & 0.73 & 0.77 & 0.178 & 3.90 & 1.48 & 10.10 \\
\quad GRU transition & 0.72 & 0.79 & 0.73 & 0.79 & 0.021 & 3.83 & 1.48 & 10.35 \\
\quad black box & -0.14 & -0.18 & 0.72 & 0.79 & 0.054 & 3.86 & 1.48 & 10.31 \\
\rowcolor{tabbase} History Transformer & -- & -- & 0.67 & 0.71 & -- & 4.03 & 1.48 & 10.21 \\
\midrule
\rowcolor{tabbase} Rain-history ridge (no model) & -- & -- & 0.72$\pm$0.03 & 0.73$\pm$0.02 & -- & -- & -- & -- \\
\bottomrule
\end{tabular}


==> tables/ms/twin_cf.tex <==
% generated by code/scripts/make_twin_table.py -- do not edit by hand
\begin{tabular}{l cccc cccc}
\toprule
\rowcolor{tabhead}  & \multicolumn{4}{c}{Direct readout} & \multicolumn{4}{c}{Probe readout} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
\rowcolor{tabhead}  & \multicolumn{2}{c}{Rain effect} & \multicolumn{2}{c}{Drydown $\tau$} & \multicolumn{2}{c}{Rain effect} & \multicolumn{2}{c}{Drydown $\tau$} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
\rowcolor{tabhead} Model & $R$ & slope & median (d) & $\rho$ & $R$ & slope & median (d) & $\rho$ \\
\midrule
\rowcolor{tabours} \method & 0.98$\pm$0.00 & 1.25$\pm$0.02 & 3.8$\pm$0.3 & 0.87$\pm$0.02 & 0.98$\pm$0.00 & 0.94$\pm$0.01 & 3.4$\pm$0.2 & 0.86$\pm$0.04 \\
\quad neural decoder & 0.05 & 0.03 & 5.3 & 0.49 & 0.98 & 0.96 & 3.2 & 0.87 \\
\quad GRU transition & 0.99 & 1.33 & 2.7 & 0.98 & 0.99 & 0.97 & 2.6 & 0.97 \\
\quad black box & -0.03 & -0.01 & 3.8 & 0.27 & 0.99 & 0.97 & 2.5 & 0.92 \\
\rowcolor{tabbase} History Transformer & -- & -- & -- & -- & 0.89 & 0.78 & 3.1 & 0.96 \\
\midrule
\rowcolor{tabbase} Rain-history ridge (no model) & -- & -- & -- & -- & 0.81$\pm$0.03 & 0.61$\pm$0.03 & 2.9$\pm$0.4 & 0.39$\pm$0.03 \\
\midrule
\rowcolor{tabbase} Truth & 1 & 1.00 & 2.7$\pm$0.3 & 1 & 1 & 1.00 & 2.7$\pm$0.3 & 1 \\
\bottomrule
\end{tabular}

